Search for Bs --> mu+ mu- at D0

We report results from a search for the decay Bs --> mu+ mu- using 1.3/fb of pbar p collisions at sqrt(s)= 1.96 TeV collected by the D0 experiment at the Fermilab Tevatron Collider. We find two candidate events, consistent with the expected background of 1.24 +/- 0.99, and set an upper limit on the branching fraction of B(Bs --> mu+ mu-) < 1.2e-7 at the 95% C.L.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            7/6/07
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\bibitem[a]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA.
\bibitem[b]{burdin}
Visitor from The University of Liverpool, Liverpool, UK.
%\bibitem[c]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA.
\bibitem[d]{podesta-lerma}
Visitor from ICN-UNAM, Mexico City, Mexico.
\bibitem[e]{quadt}
Visitor from II. Physikalisches Institut, Georg-August-University G{\"o}ttingen, Germany
\bibitem[f]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[g]{wenger}
Visitor from Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.
Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.

\bibitem[\dag]{IntFellows}
Fermilab International Fellow
\bibitem[\ddag]{deceased}
deceased

%
\vskip 0.25cm

